Anytime-valid goodness-of-fit test by $e$-spacings

To perform an anytime-valid goodness-of-fit test, we propose spacing-based $e$-processes that control the type-I error rate under arbitrary stopping rules. Based on the maximum spacing of order statistics, we construct spacing-based $e$-processes for nonparametrically testing distribution. The resulting procedures are simple and computationally efficient, and are power-consistent. We call them $e$-spacing tests. This approach is especially powerful in detecting localized discrepancy between the data-generating density and the null density. Under mild conditions, the logarithm of the proposed $e$-process is asymptotically equivalent to that of the oracle-optimal $e$-process. We further generalize the construction from maximal spacing to maximum spacing set in the form of the $1/k$ fraction of the largest $m$th order spacings, as a measure of the lower-level set of density. It boosts power under more global discrepancy from the null. Furthermore, we propose a greedy predictable scheme, via argmax or softmax rules, to combine multiple $e$-spacing testing strategies. We prove that it optimally tunes the $e$-spacing test. The proposed approach is readily generalizable to multivariate testing via a coordinate-wise Rosenblatt-transform. Simulation studies demonstrate that the proposed methods perform favorably relative to the considered anytime-valid competitors as well as various types of multiple test-adjusted Kolmogorov--Smirnov tests.

==> myPreliminary.tex <==
%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%
%%% 
%%% ### Packages 
%%%
%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%
\usepackage{varioref} 
\usepackage{xr-hyper} 
\usepackage[colorlinks]{hyperref}
\usepackage{booktabs}
\usepackage{subcaption}
\usepackage{multirow}
\RequirePackage[OT1]{fontenc}
\RequirePackage{amsthm,amsmath}
\newcommand{\hmmax}{0}
\newcommand{\bmmax}{0}
\newcommand{\under}[2][3]{\mkern#1mu\underline{\mkern-#1mu#2\mkern-#1mu}\mkern#1mu}
\usepackage{epsfig,amssymb,euscript,amsfonts,hyperref}
\usepackage{natbib} 
\usepackage{array}
\usepackage{rotating}
\usepackage{nccbbb}
\usepackage{verbatim} 
\usepackage[lined,boxed,commentsnumbered, ruled,linesnumbered]{algorithm2e}
\usepackage{graphicx}
\usepackage{float}
\usepackage{bm}
\usepackage{bbm} 
\usepackage{dsfont} 
\usepackage{MnSymbol} 
\usepackage{enumitem}
\usepackage{color}
\usepackage{caption,setspace} 
\captionsetup{font={small,stretch=1},labelfont=bf}  
\usepackage{lipsum}
\usepackage{xcolor}
\usepackage{mathbbol} 
\usepackage{marginnote}
\usepackage{forest}
\usepackage{authblk}
\usepackage{comment}
\usetikzlibrary{patterns}
\usepackage{stmaryrd}

\newcommand{\centered}[1]{\begin{tabular}{l} #1 \end{tabular}}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\numberwithin{equation}{section}

\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{H}{>{\setbox0=\hbox\bgroup}c<{\egroup}@{}}  

%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%
%%% 
%%% ### Margins
%%%
%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%	
\renewcommand{\floatpagefraction}{0.9}
\renewcommand{\topfraction}{0.95}
\renewcommand{\textfraction}{0.05}

\addtolength{\oddsidemargin}{-.5in}%
\addtolength{\evensidemargin}{-.5in}%
\addtolength{\textwidth}{1in}%
\addtolength{\textheight}{1.3in}%
\addtolength{\topmargin}{-.8in}%

\def\spacingset#1{\renewcommand{\baselinestretch}%
{#1}\small\normalsize} \spacingset{1}


%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%
%%% 
%%% ### marginnote
%%%
%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%	
\usepackage{marginnote}
\newcommand{\note}[1]{\reversemarginpar\marginnote{\tiny \hspace{-16cm}\color{myred}\setstretch{.15}\begin{minipage}{0.14\textwidth}[\textsf{KW:  #1}]\end{minipage}}}
\newcommand{\notealso}[1]{\normalmarginpar\marginnote{\tiny \color{myred}\setstretch{.35}\begin{minipage}{0.2\textwidth}[\textsf{KW:  #1}]\end{minipage}}}
\newcommand{\yunda}[1]{\textcolor{brown}{Yunda says: #1}}


%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%
%%% 
%%% ### Theorem Style
%%%
%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%	
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}

\theoremstyle{definition}
\newtheorem{example}{Example}[section]
\newtheorem{assumption}{Assumption}[section]
\newtheorem{condition}{Condition}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{model}{Model}[section]

\hypersetup{citecolor=blue}
\hypersetup{linkcolor=red}

\setcounter{equation}{0}
\setcounter{table}{0}
\setcounter{figure}{0}
\renewcommand{\theequation}{\thesection.\arabic{equation}}


%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%
%%% 
%%% ### color
%%%
%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%	
\definecolor{BUred}{rgb}{0.8, 0.0, 0.0}
\definecolor{BLUE}{rgb}{0.0, 0.28, 0.67}
\definecolor{magenta}{rgb}{1,0,.6}
\definecolor{blue0}{rgb}{0.95, 0.97, 1.0}
\definecolor{brown}{rgb}{0.75, 0.25, 0.0}

\usepackage{color}
	\definecolor{brown}{rgb}{0.75, 0.25, 0.0}
	\definecolor{mygreen}{rgb}{0.1, 0.5, 0.1}	
	\definecolor{myred}{rgb}{0.7, 0.1, 0.1}
	\definecolor{myblue}{rgb}{0.1, 0.1, 0.7}
	\definecolor{mygold}{rgb}{0.95, 0.85, 0.37}
	\definecolor{mygray}{rgb}{0.5,0.5,0.5}
	\definecolor{myorange}{rgb}{1,0.5,0}
	\definecolor{darkgreen}{RGB}{0, 100, 0}

%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%
%%% 
%%% ### \widecheck
%%%
%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%	
\usepackage{mathtools}
\makeatletter
\DeclareRobustCommand\widecheck[1]{{\mathpalette\@widecheck{#1}}}
\def\@widecheck#1#2{%
    \setbox\z@\hbox{\m@th$#1#2$}%
    \setbox\tw@\hbox{\m@th$#1%
       \widehat{%
          \vrule\@width\z@\@height\ht\z@
          \vrule\@height\z@\@width\wd\z@}$}%
    \dp\tw@-\ht\z@
    \@tempdima\ht\z@ \advance\@tempdima2\ht\tw@ \divide\@tempdima\thr@@
    \setbox\tw@\hbox{%
       \raise\@tempdima\hbox{\scalebox{1}[-1]{\lower\@tempdima\box
\tw@}}}%
    {\ooalign{\box\tw@ \cr \box\z@}}}
\makeatother

%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%
%%% 
%%% ### \widebreve
%%%
%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%	
\makeatletter
\def\widebreve{\mathpalette\wide@breve}
\def\wide@breve#1#2{\sbox\z@{$#1#2$}%
     \mathop{\vbox{\m@th\ialign{##\crcr
\kern0.08em\brevefill#1{0.8\wd\z@}\crcr\noalign{\nointerlineskip}%
                    $\hss#1#2\hss$\crcr}}}\limits}
\def\brevefill#1#2{$\m@th\sbox\tw@{$#1($}%
  \hss\resizebox{#2}{\wd\tw@}{\rotatebox[origin=c]{90}{\upshape(}}\hss$}
\makeatletter


%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%
%%% 
%%% ### Operators 
%%%
%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%	
% mathematics 
\newcommand{\diag}{\mathop{\mathrm{diag}}}
\newcommand{\vect}{\mathop{\mathrm{vec}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\KL}{\mathrm{KL}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\logit}{logit}
\DeclareMathOperator{\expit}{expit}
\newcommand{\comp}{\textsc{comp}}
\newcommand{\T}{\textsc{T}}
\newcommand{\D}{\textnormal{d}}
\newcommand{\dd}{\textnormal{d}}
\newcommand{\mathdag}{\normalfont{\dag}}


% probability 
\newcommand{\pr}{\mathsf{P}} 
\newcommand{\E}{\mathsf{E}} 
\newcommand{\median}{{\mathsf{median}}}
\newcommand{\Cov}{{\mathsf{Cov}}} 
\newcommand{\Var}{{\mathsf{Var}}}
\newcommand{\Corr}{{\mathsf{Corr}}}
\newcommand{\var}{{\mathsf{var}}}
\newcommand{\Bias}{{\mathsf{Bias}}}
\newcommand{\bias}{{\mathsf{Bias}}}
\newcommand{\Sgn}{\operatorname{\mathsf{Sgn}}}
\newcommand{\AMSE}{{\mathsf{AMSE}}}
\newcommand{\SMSE}{{\mathsf{SMSE}}}
\newcommand{\MSE}{{\mathsf{MSE}}}
\newcommand{\MSFE}{{\mathsf{MSFE}}}
\newcommand{\WMSE}{{\mathsf{WMSE}}}

% convergence and distribution relation 
\newcommand{\inD}{   \overset{ \textnormal{d}   }{\rightarrow} }
\newcommand{\inWPone}{   \overset{ \textnormal{wp1}   }{\rightarrow} }
\newcommand{\inAS}{   \overset{ \textnormal{a.s.}   }{\rightarrow} }
\newcommand{\inP}{  \overset{ \textnormal{pr}    }{\rightarrow} }
\newcommand{\inLp}{ \overset{ \mathcal{L}^p }{\rightarrow} }
%\newcommand{\indep}{\rotatebox[origin=c]{90}{$\models$}}
\newcommand{\indep}{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern4mu{#1#2}}}
\newcommand{\eqD}{   \overset{ \text{$\mathcal{D}$}   }{=} }
\newcommand{\iid}{\textsc{iid}} 
\newcommand{\simIID}{   \overset{ \iid   }{\sim} }
\newcommand{\simIND}{   \overset{ {\indep}   }{\sim} }
\newcommand{\simApprox}{   \dot{\sim} }


% statistics 
\newcommand{\RV}{\textsc{rv}}
\newcommand{\cdf}{\textsc{cdf}} 
\newcommand{\cgf}{\textsc{cgf}} 
\newcommand{\pdf}{\textsc{pdf}} 
\newcommand{\pmf}{\textsc{pmf}} 
\newcommand{\chf}{\textsc{chf}} 
\newcommand{\mgf}{\textsc{mgf}}
\newcommand{\EF}{\textsc{EF}}
\newcommand{\NEF}{\textsc{NEF}}
\newcommand{\MLE}{\textsc{MLE}}
\newcommand{\JS}{\textsc{JS}}
\newcommand{\MAP}{\textsc{MAP}}
\newcommand{\Med}{\textsc{Med}}
\newcommand{\MME}{\textsc{MME}}
\newcommand{\GMME}{\textsc{GMME}}
\newcommand{\minimax}{\textsc{M}}
\newcommand{\Bayes}{\textsc{Bayes}}
\newcommand{\Adm}{\textsc{A}}
\newcommand{\HPD}{\textsc{HPD}}
\newcommand{\ET}{\textsc{ET}}
\newcommand{\MCMC}{\textsc{mcmc}}
\newcommand{\HAC}{\textsc{hac}}
\newcommand{\AR}{\textsc{ar}}
\newcommand{\MA}{\textsc{ma}}
\newcommand{\ARMA}{\textsc{arma}}

% distribution 
\newcommand{\Bern}{\textnormal{Bern}} 
\newcommand{\WN}{\textnormal{WN}} 
\newcommand{\Unif}{\textnormal{Unif}} 
\newcommand{\Logistic}{\textnormal{Logistic}} 
\newcommand{\Normal}{\textnormal{N}} 
\newcommand{\logNormal}{\textnormal{LN}} 
\newcommand{\Bin}{\textnormal{Bin}} 
\newcommand{\NB}{\textnormal{NB}} 
\newcommand{\HG}{\textnormal{HG}} 
\newcommand{\Geom}{\textnormal{Geom}} 
\newcommand{\Beta}{\textnormal{Beta}} 
\newcommand{\BetaBin}{\textnormal{Beta-Bin}}
\newcommand{\Ga}{\textnormal{Ga}} 
\newcommand{\Exp}{\textnormal{Exp}}
\newcommand{\Gam}{\textnormal{Gamma}}
\newcommand{\Expo}{\textnormal{Expo}} 
\newcommand{\Po}{\textnormal{Po}} 
\newcommand{\Multi}{\textnormal{Multi}} 
\newcommand{\Wishart}{\textnormal{Wishart}} 
\newcommand{\MIG}{\textnormal{MIG}} 
\newcommand{\student}{\textnormal{t}} 
\newcommand{\Cauchy}{\textnormal{Cauchy}} 
\newcommand{\Pareto}{\textnormal{Pareto}} 
\newcommand{\Laplace}{\textnormal{Laplace}} 
\newcommand{\Dir}{\textnormal{Dir}} 
\newcommand{\DP}{\textnormal{DP}} 
\newcommand{\Inv}{\textnormal{Inv-}} 
\newcommand{\F}{\textnormal{F}} 

% e-spacings
\newcommand{\cH}{\ensuremath{\mathcal H}}
\newcommand{\md}{(1,\infty)}
\newcommand{\agg}{{}}  %\mathsf{gen}
\newcommand{\para}{\mathsf{para}}
\newcommand{\npara}{\mathsf{npara}}
\newcommand{\pilot}{\wp}
\newcommand{\AS}{\textnormal{a.s.}} 
\newcommand{\Leb}{\textnormal{Leb}} 
\newcommand{\Supp}{\textnormal{Supp}} 
\newcommand{\round}{\textnormal{round}} 












